Strong Screening Rules for Group-based SLOPE Models

Tuning the regularization parameter in penalized regression models is an expensive task, requiring multiple models to be fit along a path of parameters. Strong screening rules drastically reduce computational costs by lowering the dimensionality of the input prior to fitting. We develop strong screening rules for group-based Sorted L-One Penalized Estimation (SLOPE) models: Group SLOPE and Sparse-group SLOPE. The developed rules are applicable to the wider family of group-based OWL models, including OSCAR. Our experiments on both synthetic and real data show that the screening rules significantly accelerate the fitting process. The screening rules make it accessible for group SLOPE and sparse-group SLOPE to be applied to high-dimensional datasets, particularly those encountered in genetics.

==> new_sections/1-introduction.tex <==
As the amount of data collected increases, the emergence of high-dimensional data, where the number of features ($p$) is much larger than the number of observations ($n$), is becoming increasingly common in fields ranging from genetics to finance. Performing regression and discovering relevant features on these datasets is a challenging task, as classical statistical methods tend to break down. The most popular approach to meeting this challenge is the \textit{Lasso} \citep{Tibshirani1996RegressionLasso}, which has given rise to the general penalized regression framework
\begin{equation}\label{eqn:general_problem}
    \hat\beta(\lambda) = \argmin_{\beta \in \mathbb{R}^p} \left\{ f(\beta)+\lambda J(\beta;v)\right\},
\end{equation}
where $f$ is the loss function, $J$ is a convex penalty norm, $v \succeq 0$ are penalty parameters, and $\lambda>0$ is the regularization parameter. 

A key aspect of fitting a penalized model is to tune the value of the regularization parameter, which determines the level of sparsity in the fitted model. Several approaches exist in the literature for fitting these models, which are beyond the scope of this manuscript. The focus of this manuscript is screening rules, that reduce the dimensions of the input dimensionality by discarding irrelevant features before the fitting process. Discarding features, especially in high-dimensional settings has a tremendous impact on the computational costs. 


Denoting the \textit{active set} of non-zero parameters at $\lambda_{k+1}$ by $\mathcal{A}_v(\lambda_{k+1}) = \{i \in \{1,\dots,p\}:\hat\beta_i(\lambda_{k+1})\neq 0\}$, the goal of a screening rule is to use the solution at $\lambda_k$ to recover a \textit{screened set} of features, $\mathcal{S}_v(\lambda_{k+1})$, which is a superset of $\mathcal{A}_v(\lambda_{k+1})$. The screened set can then be used as input for calculating the fitted values. By finding the smallest possible screened set, that still contains the active set, the number of irrelevant features included in the fitting process is reduced.

There are two types of screening rules: \textit{safe} and \textit{heuristic}. Safe rules, as suggested by the name, provide guarantees that any variables discarded are in fact inactive at the solution. The seminal work of \citep{Ghaoui2010SafeProblems} introduced the Safe Feature Elimination Rule (SAFE) for the lasso, in which safe regions were constructed to eliminate non-active features. Other examples of safe rules are given by \citep{pmlr-v28-ogawa13b, pmlr-v119-atamturk20a, Wang2013LassoProjection}, including sample screening by \citep{Shibagaki2016}. Heuristic rules, on the other hand, tend to discard more variables, but this increased screening efficiency can lead to active variables being incorrectly discarded. Examples of heuristic screening rules are given in \citep{Fan2008, tibshirani2010strong, AHMED201933}. Amongst the proposed heuristic rules, of particular interest is the
strong screening rule framework developed for the lasso by \citep{tibshirani2010strong}. As strong screening rules can lead to violations, \cite{tibshirani2010strong} complemented their rules with a check of the Karush–Kuhn–Tucker (KKT) \citep{Kuhn1950NonlinearProgramming} optimality conditions to ensure no such violations occur. 
Hybrid screening regimes that combine safe and heuristic rules have recently been proposed in the literature \citep{Zeng2021,Wang2022}.
%There have been attempts to combine safe and heuristic rules, leading to hybrid screening regimes \cite{Zeng2021,Wang2022}.
%However, screening rules for adaptive extensions to the lasso are rarer. }
%Strong screening rules are broken down into sequential and basic rules. A sequential rule is applied to a path of regularization parameters. As a basic rule is a generalisation of a sequential rule, we only consider sequential rules in this paper. 

The strong screening rule is formulated by computing the KKT conditions for Equation \ref{eqn:general_problem}, given by:
\begin{equation}\label{eqn:kkt_condition}
    \mathbf{0} \in \nabla f(\beta) + \lambda\partial J(\beta;v).
\end{equation}
If the gradient, $\nabla f(\hat\beta(\lambda_{k+1}))$, was available, the set $\mathcal{A}_v(\lambda_{k+1})$ could be identified by checking the subdifferential of the norm at zero. That is, checking for which variables 
\begin{equation}\label{eqn:subdiff_at_zero}
    -\nabla f(\beta) \in \lambda \partial J(\mathbf{0};v) = \{x : J^*(x;\lambda v) \leq 1\},
\end{equation}
where $J^*$ refers to the dual norm of $J$. The subdifferential at zero, $\partial J(\mathbf{0};v)$, can also be seen to be the unit ball of its dual norm. As the gradient at $\lambda_{k+1}$ is not available in practice, an approximation of the gradient is used to find a screened subset of the features, $\mathcal{S}_v(\lambda_{k+1})$. The screened variables are combined with the previously active ones to form the reduced input space, $\mathcal{E}_v(\lambda_{k+1}) = \mathcal{S}_v(\lambda_{k+1})\cup \mathcal{A}_v(\lambda_k)$. The fitted values are then calculated by solving Equation \ref{eqn:general_problem} using only the variables in $\mathcal{E}_v(\lambda_{k+1})$. Optimality of the fitted values is checked for using the KKT conditions (Equation \ref{eqn:kkt_condition}), with violations added into $\mathcal{E}_v$. This ensures features are not discarded that should be active. Strong screening rules are usually time efficient as the extra cost of the screening algorithm and KKT checks tend to be outweighed by the significant savings of fitting on a reduced input space.

%Strong screening rules are usually time efficient as the extra cost of the screening algorithm and KKT checks tend to be outweighed by the significant savings of fitting on a reduced input space. Given the above outlined advantages of the strong screening rules, in this manuscript, we have focused on the development of strong screening rules for group-based models.

Over the years, several adaptive extensions to the lasso have been proposed, including the  \textit{Sorted L-One Penalized Estimation} (\textit{SLOPE}) method \citep{Bogdan2015SLOPEAdaptiveOptimization}. SLOPE applies the sorted $\ell_1$ norm $J_\text{slope}(\beta;v) = \sum_{i=1}^p v_i|\beta|_{(i)}$, where $v_1 \geq \ldots \geq v_p \geq 0, |\beta|_{(1)}\geq \ldots \geq |\beta|_{(p)}$. One key advantage of SLOPE is its ability to control the variable false discovery rate (FDR) under orthogonal data. Both safe and strong rules have been proposed in the literature for SLOPE \citep{Bao2020FastRules,Larsson2020a,Elvira2021SafeProblem}, as well as an exact solution path algorithms \citep{Nomura2020,Dupuis2023}. As SLOPE is a non-separable penalty, safe screening rules require repeated screening during the fitting process \citep{Larsson2020a}. This tends to be a computational bottleneck, as the calculation of the safe regions required for screening can be expensive.

\subsection{Contributions} 
Strong screening rules are time efficient as the extra cost of the screening algorithm and KKT checks tend to be outweighed by the significant savings of fitting on a reduced input space. Motivated by this result, strong screening rules are introduced for the first time for two group-based extensions of SLOPE: \textit{Group SLOPE} (\textit{gSLOPE}) \citep{Brzyski2019GroupPredictors} and \textit{Sparse-group SLOPE} (\textit{SGS}) \citep{Feser2023Sparse-groupFDR-control}. 

Both of these approaches were developed for the analysis of features that naturally belong to groups. For example, this is situation frequently encountered in the analysis of genetics data, where genes are grouped into pathways (gene sets) for the completion of a specific biological task. The gSLOPE approach selects groups of features, whereas SGS performs bi-level selection, by applying penalization at both variable and group levels. Both approaches have been shown to inherit SLOPE's ability to control FDR under orthogonal data. gSLOPE is able to control group FDR \citep{Brzyski2019GroupPredictors} and SGS offers both variable and group FDR-control \citep{Feser2023Sparse-groupFDR-control}. 

Section \ref{sec:framework} introduces a sparse-group screening rule framework. Based on this, strong screening rules for gSLOPE and SGS are developed and presented in Sections \ref{sec:gSLOPE} and \ref{sec:SGS}. 

%For penalized regression models, tuning the regularization parameter is of high importance, as its value determines the level of sparsity in the fitted model. For the SLOPE family of models, this is particularly important as the level of sparsity determines the FDR of the estimates. Being able to run a model faster allows for an expanded tuning regime, giving greater control over the FDR. 

Through a series of simulations and the analysis of real datasets, the proposed screening rules are shown to significantly reduce computational runtime. Additionally, due to the reduced input dimensionality offered by screening rules, issues with convergence in the analysis of large datasets are shown to be alleviated. These improvements are achieved without affecting the accuracy of the methods. 


%For such situations, group and sparse-group regression models have proven useful. SLOPE has been extended to the group and sparse-group regression settings through \textit{Group SLOPE} (\textit{gSLOPE}) \cite{Brzyski2019GroupPredictors} and \textit{Sparse-Group SLOPE} (\textit{SGS}) \cite{Feser2023Sparse-groupFDR-control}. Both these approaches have been shown to inherit SLOPE's ability to control FDR under orthogonal data, such that gSLOPE is able to control group FDR \citep{Brzyski2019GroupPredictors} and SGS offers both variable and group FDR control \citep{Feser2023Sparse-groupFDR-control}.


%Both safe and strong rules have previously been proposed in the literature for SLOPE .  As SLOPE is a non-separable penalty, safe screening rules tend to require repeated screening during the fitting process, whereas strong screening rules do not and hence are preferred \cite{Larsson2020a}. 
%Safe screening rules for SLOPE have been proposed in \cite{Bao2020FastRules,Elvira2021SafeProblem}. A strong screening rule for SLOPE has been proposed in \cite{Larsson2020a}.

\subsection{Notation}
Throughout this manuscript the following notation is used. We assume that our feature space is divided into a set of $m$ groups, where $\mathcal{G}_1,\dots,\mathcal{G}_m$ denote the set of variable indices for each group. The set of active groups is denoted by $\mathcal{A}_g = \{i \in \{1,\dots,m\}: \|\hat\beta^{(i)}\|_2\neq 0\}$ whereas $\mathcal{Z} = \{i \in \{1,\dots,m\}: \|\hat\beta^{(i)}\|_2= 0\}$ presents the inactive groups. The set of variable indices of the active and inactive groups are denoted by $\mathcal{G}_\mathcal{A}$ and $\mathcal{G}_\mathcal{Z}$, respectively. 

The cardinality of a vector $x$ is denoted by $\card(x)$, and the operator $(\cdot)_\downarrow$ sorts a vector into decreasing form. The $\preceq$ is the element-wise less than or equal to operator. The operator $\mathcal{O}(\cdot)$ returns the index of a vector sorted in decreasing form by absolute value. The cumulative summation operator applied on a vector is denoted by $\text{cumsum}(x) = [x_1,x_1+x_2,\ldots, \sum_{i=1}^{\card(x)} x_i]$. 


==> new_sections/old_kkt.tex <==
as the additional layer of screening carries with it additional assumptions. Additionally, the subdifferential term in Equation \ref{eqn:group_condition_sgs} was chosen to be as small as possible, leading to tighter screened sets. The increased violations are reflective of this. On both the simulated and real datasets, SGS recorded an increasing number of KKT violations as the fitted models became denser (Figure Figures \ref{fig:kkt_spikeplot_synth} and \ref{fig:kkt_spikeplot}). The shape of the increasing number of KKT violations mirrors the log-linear shape of the regularization path. The trend of increasing KKT violations with denser models is also observed for the SLOPE strong screening rule \citep{Larsson2020a}.

Despite the increased number of KKT violations for SGS, which amounts to the additional computational cost of performing the KKT checks and repeated sub-fitting in Algorithm \ref{alg:sgs_framework}, the overall screening procedure still results in substantial runtime improvements, as evidenced in Tables \ref{tbl:sim_data} and \ref{tbl:real_data_sizes}. This shows that screening rules can provide improvements to computational cost, even with assumptions that are often violated.



For SGS, KKT violations are more common (Figures \ref{fig:kkt_spikeplot_synth} and \ref{fig:kkt_spikeplot}), as the second layer of screening requires additional assumptions. Additionally, in Equation \ref{eqn:group_condition_sgs}, the subdifferential term was taken to be as small as possible, leading to tighter screened sets. The increased violations are reflective of this.  

On both the simulated and real datasets, SGS recorded an increasing number of KKT violations as the fitted models became denser (Figures \ref{fig:kkt_spikeplot_synth} and \ref{fig:kkt_spikeplot}). The shape of the increasing number of KKT violations mirrors the log-linear shape of the regularization path. The trend of increasing KKT violations with denser models is also observed for the SLOPE strong screening rule \citep{Larsson2020a}.

Despite the increased number of KKT violations for SGS, which amounts to the additional computational cost of performing the KKT checks and repeated sub-fitting in Algorithm \ref{alg:sgs_framework}, the overall screening procedure still results in substantial runtime improvements, as evidenced by our results, where screening was found to provide a benefit in every situation considered (Tables \ref{tbl:sim_data} and \ref{tbl:real_data_sizes}). 

